On-device Content-based Recommendation with Single-shot Embedding Pruning: A Cooperative Game Perspective

Content-based Recommender Systems (CRSs) play a crucial role in shaping user experiences in e-commerce, online advertising, and personalized recommendations. However, due to the vast amount of categorical features, the embedding tables used in CRS models pose a significant storage bottleneck for real-world deployment, especially on resource-constrained devices. To address this problem, various embedding pruning methods have been proposed, but most existing ones require expensive retraining steps for each target parameter budget, leading to enormous computation costs. In reality, this computation cost is a major hurdle in real-world applications with diverse storage requirements, such as federated learning and streaming settings. In this paper, we propose Shapley Value-guided Embedding Reduction (Shaver) as our response. With Shaver, we view the problem from a cooperative game perspective, and quantify each embedding parameter's contribution with Shapley values to facilitate contribution-based parameter pruning. To address the inherently high computation costs of Shapley values, we propose an efficient and unbiased method to estimate Shapley values of a CRS's embedding parameters. Moreover, in the pruning stage, we put forward a field-aware codebook to mitigate the information loss in the traditional zero-out treatment. Through extensive experiments on three real-world datasets, Shaver has demonstrated competitive performance with lightweight recommendation models across various parameter budgets. The source code is available at https://github.com/chenxing1999/shaver

==> figures/rq1/data/avazu.tex <==
\renewcommand{\arraystretch}{0.8}
\begin{table*}[th]
    \centering
\begin{tabular}{llrrlrrlrrl}
    \toprule
    & \multirow[c]{1}{*}{Sparsity Rate} & \multicolumn{3}{c}{50\%} & \multicolumn{3}{c}{80\%} & \multicolumn{3}{c}{95\%} \\
    \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
     % Backbone & Method & AUC ($\uparrow$) & Loss ($\downarrow$) & Params & AUC ($\uparrow$) & Loss ($\downarrow$) & Params & AUC ($\uparrow$) & Loss ($\downarrow$) & Params \\
     Backbone & Method & AUC & Loss & Params & AUC & Loss & Params & AUC & Loss & Params \\
     % Backbone & Method & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Loss} & \multicolumn{1}{c}{Params} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Loss} & \multicolumn{1}{c}{Params} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Loss} & \multicolumn{1}{c}{Params} \\
    \midrule

\multirow[c]{11}{*}{DeepFM} 
 % & DHE & 0.7554 & 0.3959 & 31.74M & 0.7536 & 0.3957 & 14.74M & 0.7601 & 0.3964 & 3.35M \\
     & QR \cite{qr2019} & \underline{0.7697} & \underline{0.3864} & 35.43M & \underline{0.7695} & \underline{0.3871} & 14.17M & \underline{0.7644} & \underline{0.3905} & 3.54M \\
  & TTRec \cite{ttrec2021} & 0.7647 & 0.3915 & 35.43M & 0.7651 & 0.3902 & 14.17M & 0.7608 & 0.3924 & 3.54M \\
   & PEP \cite{pep2021} & 0.7647 & 0.3886 & 29.67M & 0.7633 & 0.3896 & 14.07M & 0.7590 & 0.3922 & 3.50M \\
   & OptEmb \cite{optembed2022} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 0.7585 & 0.3936 & 3.41M \\
& CERP \cite{cerp2023} & 0.7649 & 0.3885 & 35.30M & 0.7638 & 0.3892 & 14.14M & 0.7607 & 0.3920 & 3.54M \\

 & MagPrune \cite{tran2024thorough} & 0.7655 & 0.3932 & 35.43M & 0.7604 & 0.3962 & 14.17M & 0.7501 & 0.4034 & 3.54M \\

\cmidrule(lr){2-11}
 & Shaver-Zero & 0.7655 & 0.3934 & 35.43M & 0.7645 & 0.3942 & 14.17M & 0.7575 & 0.3984 & 3.54M \\
 & Shaver-Zero$\dagger$ & \textbf{0.7715} & \textbf{0.3855} & 35.43M & \textbf{0.7715} & \textbf{0.3857} & 14.17M & \textbf{0.7655} & \textbf{0.3902} & 3.54M \\
  & Shaver-Codebook & 0.7647 & 0.3939 & 35.43M & 0.7623 & 0.3952 & 14.17M & 0.7543 & 0.4002 & 3.54M \\
 & Shaver-Codebook$\dagger$ & 0.7644 & 0.3903 & 35.43M & 0.7602 & 0.3940 & 14.17M & 0.7552 & 0.3974 & 3.54M \\

\midrule
    
\multirow[c]{11}{*}{DCN - Mix} 
   & QR \cite{qr2019} & 0.7743 & 0.3857 & 35.43M & 0.7698 & 0.3922 & 14.17M & 0.7652 & 0.3895 & 3.54M \\
 & TTRec \cite{ttrec2021} & 0.7711 & 0.3873 & 35.43M & 0.7710 & 0.3900 & 14.17M & 0.7678 & 0.3903 & 3.54M \\
 & PEP \cite{pep2021} & 0.7754 & 0.3852 & 33.55M & 0.7669 & 0.3906 & 12.57M & 0.7564 & 0.3938 & 3.52M \\
 & OptEmb \cite{optembed2022} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 0.7663 & 0.3877 & 13.24M & 0.7683 & 0.3895 & 3.43M \\
 & CERP \cite{cerp2023} & 0.7723 & 0.3852 & 35.34M & 0.7673 & 0.3873 & 13.05M & 0.7631 & 0.3933 & 3.54M \\
 & MagPrune \cite{tran2024thorough} & 0.7754 & 0.3841 & 35.43M & 0.7713 & 0.3862 & 14.17M & 0.7602 & 0.3924 & 3.54M \\
 
\cmidrule(lr){2-11}

 & Shaver-Zero & 0.7759 & 0.3837 & 35.43M & \underline{0.7745} & \textbf{0.3840} & 14.17M & \underline{0.7690} & \textbf{0.3865} & 3.54M \\
 & Shaver-Zero$\dagger$ & \underline{0.7777} & \underline{0.3817} & 35.43M & 0.7735 & 0.3849 & 14.17M & \textbf{0.7703} & \underline{0.3868} & 3.54M \\
  & Shaver-Codebook & 0.7762 & 0.3838 & 35.43M & \textbf{0.7749} & \underline{0.3842} & 14.17M & 0.7683 & 0.3873 & 3.54M \\
 & Shaver-Codebook$\dagger$ & \textbf{0.7781} & \textbf{0.3816} & 35.43M & 0.7717 & 0.3870 & 14.17M & 0.7670 & 0.3952 & 3.54M \\
 
% \vspace{-0.35cm}\\
\cline{1-11}

\bottomrule
\end{tabular}
    \caption{Results on the Avazu dataset. \textmd{The sparsity $t$ indicates the number of pruned parameters (the higher $t$ is, the more parameters are reduced). ``Params'' indicates the parameter size of the embedding table (M: million). $\dagger$ denotes fine-tuned models after pruned. In each column, the best result is marked in bold and the second best one is underlined. ``-'' indicates not converging.}}
    \label{tab:avazu-exp}
\end{table*}
\renewcommand{\arraystretch}{1.0}


==> figures/rq1/data/criteo.tex <==
\renewcommand{\arraystretch}{0.8}
\begin{table*}[th]
    \centering
    \caption{Results on the Criteo dataset. \textmd{The sparsity $t$ indicates the number of pruned parameters (the higher $t$ is, the more parameters are reduced). ``Params'' indicates the parameter size of the embedding table (M: million, K: thousand). $\dagger$ denotes fine-tuned models after pruned. In each column, the best result is marked in bold and the second best one is underlined. ``-'' indicates not converging.}}
    \vspace{-.3cm}
    \begin{tabular}{llrrlrrlrrl}
    \toprule
    & \multirow[c]{1}{*}{Sparsity Rate} & \multicolumn{3}{c}{50\%} & \multicolumn{3}{c}{80\%} & \multicolumn{3}{c}{95\%} \\
    \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
     Backbone & Method & AUC & Loss & Params & AUC & Loss & Params & AUC & Loss & Params \\
    % Backbone & Method & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Loss} & \multicolumn{1}{c}{Params} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Loss} & \multicolumn{1}{c}{Params} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Loss} & \multicolumn{1}{c}{Params} \\
    \midrule
    \multirow[c]{11}{*}{DeepFM} 
    
     % & DHE & 0.8050 & 0.4467 & 8.69M & 0.8053 & 0.4463 & 3.17M & 0.8050 & 0.4466 & 846K \\
     & QR \cite{qr2019} & 0.8081 & 0.4435 & 8.69M & 0.8078 & 0.4438 & 3.48M & 0.8033 & 0.4482 & 870K \\
     & TTRec \cite{ttrec2021} & 0.8075 & 0.4442 & 9.36M & 0.8070 & 0.4446 & 3.15M & 0.8087 & 0.4431 & 870K \\
     & PEP \cite{pep2021} & \textbf{0.8105} & \textbf{0.4414} & 8.67M & 0.8098 & 0.4419 & 3.47M & 0.8084 & 0.4432 & 806K \\
     & OptEmb \cite{optembed2022} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 0.8088 & 0.4430 & 3.17M & 0.8043 & 0.4471 & 863K \\
     & CERP \cite{cerp2023} & 0.8099 & 0.4419 & 8.66M & 0.8095 & 0.4423 & 3.21M & 0.8062 & 0.4454 & 864K \\
     & MagPrune \cite{tran2024thorough} & 0.8102 & 0.4417 & 8.69M & 0.8101 & 0.4417 & 3.48M & 0.8080 & 0.4436 & 869K \\
     \cmidrule(lr){2-11}
     & Shaver-Zero & 0.8101 & 0.4417 & 8.69M & 0.8100 & 0.4418 & 3.48M & 0.8085 & 0.4432 & 869K \\
     & Shaver-Zero$\dagger$ & 0.8103 & 0.4415 & 8.69M & \textbf{0.8105} & \textbf{0.4414} & 3.48M & \underline{0.8104} & \underline{0.4414} & 869K \\
      & Shaver-Codebook & 0.8101 & 0.4417 & 8.69M & 0.8101 & 0.4418 & 3.48M & 0.8093 & 0.4425 & 870K \\
     & Shaver-Codebook$\dagger$ & \textbf{0.8105} & \textbf{0.4414} & 8.69M & \textbf{0.8105} & \textbf{0.4414} & 3.48M & \textbf{0.8106} & \textbf{0.4413} & 870K \\
    % \cline{1-11}
    \midrule
    \multirow[c]{11}{*}{DCN-Mix} 
     & QR \cite{qr2019} & 0.8095 & 0.4425 & 8.69M & 0.8091 & 0.4427 & 3.48M & 0.8064 & 0.4452 & 870K \\
     % & DHE & 0.8095 & 0.4427 & 8.69M & 0.8109 & 0.4412 & 3.17M & 0.8098 & 0.4420 & 846K \\
     & TTRec \cite{ttrec2021} & 0.8112 & 0.4408 & 8.26M & 0.8103 & 0.4416 & 3.48M & 0.8106 & 0.4414 & 870K \\
     & PEP \cite{pep2021} & 0.8113 & 0.4407 & 8.69M & 0.8108 & 0.4413 & 3.46M & \textbf{0.8114} & \textbf{0.4406} & 831K \\
     & OptEmb \cite{optembed2022} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 0.8112 & 0.4408 & 1.45M & 0.8109 & 0.4408 & 856K \\
     & CERP \cite{cerp2023} & 0.8110 & 0.4410 & 8.66M & 0.8106 & 0.4416 & 3.44M & 0.8107 & 0.4414 & 850K \\
     & MagPrune \cite{tran2024thorough} & 0.8113 & 0.4407 & 8.69M & 0.8111 & 0.4410 & 3.48M & 0.8086 & 0.4434 & 869K \\
     \cmidrule(lr){2-11}
     & Shaver-Zero & 0.8114 & 0.4407 & 8.69M & \textbf{0.8114} & \textbf{0.4407} & 3.48M & 0.8110 & 0.4412 & 869K \\
     & Shaver-Zero$\dagger$ & \textbf{0.8116} & \textbf{0.4404} & 8.69M & \textbf{0.8114} & \textbf{0.4407} & 3.48M & \underline{0.8112} & \underline{0.4409} & 869K \\
      & Shaver-Codebook & 0.8114 & 0.4407 & 8.69M & \textbf{0.8114} & \textbf{0.4407} & 3.48M & \underline{0.8112} & 0.4410 & 870K \\
     & Shaver-Codebook$\dagger$ & \underline{0.8115} & \underline{0.4405} & 8.69M & \textbf{0.8114} & \textbf{0.4407} & 3.48M & \underline{0.8112} & 0.4410 & 870K \\
    
    % \vspace{-0.25cm}\\
    % \cline{1-11}

    \bottomrule
    \end{tabular}
    \vspace{-.2cm}

    \label{tab:criteo-exp}
\end{table*}


\renewcommand{\arraystretch}{1.0} % Reset row spacing


==> figures/rq1/data/kdd.tex <==
\renewcommand{\arraystretch}{0.8}
\begin{table*}[pth]
    \centering
        \caption{Results on the KDD dataset. \textmd{The sparsity $t$ indicates the number of pruned parameters (the higher $t$ is, the more parameters are reduced). ``Params'' indicates the parameter size of the embedding table (M: million). $\dagger$ denotes fine-tuned models after pruned. In each column, the best result is marked in bold and the second best one is underlined.}}
    \vspace{-.3cm}
\begin{tabular}{llrrlrrlrrl}
    \toprule
    & \multirow[c]{1}{*}{Sparsity Rate} & \multicolumn{3}{c}{50\%} & \multicolumn{3}{c}{80\%} & \multicolumn{3}{c}{95\%} \\
    \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
     % Backbone & Method & AUC ($\uparrow$) & Loss ($\downarrow$) & Params & AUC ($\uparrow$) & Loss ($\downarrow$) & Params & AUC ($\uparrow$) & Loss ($\downarrow$) & Params \\
     Backbone & Method & AUC & Loss & Params & AUC & Loss & Params & AUC & Loss & Params \\
  % Backbone & Method & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Loss} & \multicolumn{1}{c}{Params} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Loss} & \multicolumn{1}{c}{Params} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Loss} & \multicolumn{1}{c}{Params} \\
    \midrule

\multirow[c]{11}{*}{DeepFM} 
 % & DHE & 0.7554 & 0.3959 & 31.74M & 0.7536 & 0.3957 & 14.74M & 0.7601 & 0.3964 & 3.35M \\
 & QR \cite{qr2019} & 0.7744 & 0.1579 & 48.16M & 0.7753 & 0.1578 & 19.26M & 0.7779 & 0.1573 & 4.82M \\
  & TTRec \cite{ttrec2021} & 0.7762 & 0.1588 & 48.16M & 0.7727 & 0.1583 & 19.26M & \underline{0.7785} & \underline{0.1572} & 4.82M \\
   & PEP \cite{pep2021} & 0.7801 & 0.1568 & 47.80M & 0.7745 & 0.1578 & 19.22M & 0.7730 & 0.1579 & 4.71M  \\
   & OptEmb \cite{optembed2022} & 0.7742 & 0.1584 & 47.52M & 0.7740 & 0.1584 & 18.29M
   & 0.7663 & 0.1597 & 4.79M  
   \\
& CERP \cite{cerp2023} & 0.7818 & 0.1567 & 48.10M & 0.7765 & 0.1578 & 18.57M & 0.7727 & 0.1581 & 4.77M \\

 & MagPrune \cite{tran2024thorough} & 0.7827 & 0.1568 & 48.16M & 0.7759 & 0.1577 & 19.26M & 0.7597 & 0.1609 &  4.82M\\

\cmidrule(lr){2-11}
 & Shaver-Zero & \underline{0.7846} & \underline{0.1563} & 48.16M  & \underline{0.7836} & \underline{0.1565} & 19.26M & 0.7766 & 0.1578 &  4.82M\\
 & Shaver-Zero$\dagger$ & \underline{0.7846} & \underline{0.1563} & 48.16M & \underline{0.7836} & \underline{0.1565} & 19.26M & 0.7766 & 0.1578 & 4.82M\\
  & Shaver-Codebook & \textbf{0.7850} & \textbf{0.1562} & 48.16M & \textbf{0.7854} & \textbf{0.1560} & 19.26M & \textbf{0.7812} & \textbf{0.1567} & 4.82M\\
 & Shaver-Codebook$\dagger$ & \textbf{0.7850} & \textbf{0.1562} & 48.16M & \textbf{0.7854} & \textbf{0.1560} & 19.26M & \textbf{0.7812} & \textbf{0.1567} & 4.82M \\

\midrule

\multirow[c]{11}{*}{DCN - Mix} 

 % & DHE & 0.7594 & 0.3921 & 31.74M & 0.7650 & 0.3916 & 14.74M & 0.7677 & 0.3913 & 3.35M \\

   & QR \cite{qr2019} & 0.7724 & 0.1581 & 48.16M & 0.7709 & 0.1584 & 19.26M & 0.7702 & 0.1588 & 4.82M \\
 & TTRec \cite{ttrec2021} & 0.7862 & 0.1576 & 48.16M & \underline{0.7843} & \underline{0.1564} & 19.26M & 0.7815 & \textbf{0.1559} & 4.82M \\
 & PEP \cite{pep2021} & 0.7754 & 0.1576 & 45.93M & 0.7731 & 0.1581 & 18.88M & 0.7737 & 0.1579 & 4.50M \\
 & OptEmb \cite{optembed2022} & \textbf{0.7877} & \textbf{0.1558} & 48.99M  
 & 0.7818 & 0.1593 & 15.10M & \underline{0.7826} & 0.1591 & 4.80M\\
 & CERP \cite{cerp2023} & 0.7841 & 0.1566 & 47.50M & 0.7781 & 0.1573 & 19.18M & 0.7721 & 0.1589 & 4.68M \\
 & MagPrune \cite{tran2024thorough} & 0.7822 & 0.1569 & 48.16M & 0.7649  & 0.1598 & 19.26M & 0.7469 & 0.1728 & 4.82M \\
 
\cmidrule(lr){2-11}

 & Shaver-Zero & 0.7858 & 0.1563 & 48.16M & 0.7826 & 0.1569 & 19.26M & 0.7699 & 0.1601 & 4.82M \\
 & Shaver-Zero$\dagger$ & 0.7858 & 0.1563 & 48.16M & 0.7826 & 0.1569 & 19.26M & 0.7775 & 0.1576 & 4.82M \\
  & Shaver-Codebook & \underline{0.7870} & \underline{0.1559} & 48.16M & \textbf{0.7870} & \textbf{0.1557} & 19.26M & \textbf{0.7836} & \underline{0.1563} & 4.82M \\
 & Shaver-Codebook$\dagger$ & 0.7754 & 0.1608 & 48.16M &  0.7806 & 0.1625 & 19.26M & 0.7836 & 0.1563  & 4.82M \\
 
% \vspace{-0.35cm}\\
% \cline{1-11}

\bottomrule
\end{tabular}
    \vspace{-.3cm}

\label{tab:kdd-exp}
\end{table*}
\renewcommand{\arraystretch}{1.0}

%Note: KDD OptEmbed use Linear scale until 95%
% try exp scale latex

==> figures/rq1/performance-table-no-taylor.tex <==
\begin{table*}[t!]
    \centering
% \renewcommand{\arraystretch}{1.2}
\setlength\tabcolsep{3pt}
\caption{Results on CTR prediction with DeepFM and DCN as the base models. The sparsity $t$ indicates the number of pruned parameters (the higher $t$ is, the more parameters are reduced). \#Para indicates the parameter size of the embedding table (M: million, K: thousand). $\dagger$ denotes fine-tuned models after pruned. In each column, the best result is marked in bold and the second best one is underlined.}
\vspace{-0.2cm}
\begin{tabular}{cl|llr llr|llr llr}
\hline
    & & \multicolumn{6}{c|}{Criteo} & \multicolumn{6}{c}{Avazu} \\
\cline{3-14}
    & & \multicolumn{3}{c}{DeepFM} & \multicolumn{3}{c|}{DCN} & \multicolumn{3}{c}{DeepFM} & \multicolumn{3}{c}{DCN} \\
\cline{3-14}
     Sparsity    & Method &  AUC      & Loss & \#Param  &  AUC      & Loss & \#Param  & AUC      & Loss & \#Param &  AUC      & Loss & \#Param \\
\cline{1-14}
    0\% & Original & 0.8102 & 0.4416 & 17.39M & 0.8114 & 0.4407 & 17.39M 
                   & 0.7658 & 0.3932 & 70.86M & 0.7759 & 0.3839 & 70.86M \\
\cline{1-14}
 -\% & OptEmb & 0.8088 & 0.4429 & 4.41M & 0.8112 & 0.4408 & 1.45M 
                & 0.7585 & 0.3936 & 3.41M & 0.7671 & 0.3878 & 19.81M \\
\cline{1-14}
\multirow{12}{*}{$\sim 50\%$} % update 6 to 6 + 6 = 12
& QR \cite{qr2019}       & 0.8081  & 0.4435 & 8.69M & 0.8095 & 0.4425 & 8.69M 
                        & \underline{0.7697}  & \underline{0.3864} & 35.43M & 0.7743 & 0.3857 & 35.43M           \\
& TTRec \cite{ttrec2021} & 0.8075  & 0.4442 & 9.36M & 0.8112 & 0.4408 & 8.26M
                        & 0.7647  & 0.3915 & 35.43M & 0.7711 & 0.3873 & 35.43M         \\
& DHE \cite{dhe2021}     & 0.8050  & 0.4467 & 8.69M & 0.8095 & 0.4427 & 8.69M
                        & 0.7554  & 0.3959 & 31.74M & 0.7594 & 0.3921 & 31.74M         \\
& PEP \cite{pep2021}     & \textbf{0.8105} & \textbf{0.4414} & 8.67M & 0.8113 & 0.4407 & 8.69M
                        & 0.7647 & 0.3886  & 29.67M  & 0.7754 & 0.3852 & 33.55M      \\
& CERP \cite{cerp2023}   & 0.8099  & 0.4419  & 8.66M  & 0.8110 & 0.4410 & 8.66M       
                        & 0.7649 & 0.3885 & 35.30M & 0.7723 & 0.3852 & 35.34M     \\
& MagPrune \cite{tran2024thorough}              & 0.8102  & 0.4417 & 8.69M & 0.8113 & 0.4407 & 8.69M
                        & 0.7655  & 0.3932 & 35.43M & 0.7754 & 0.3841 & 35.43M          \\
% & Taylor                & 0.8102 & 0.4416 & 8.69M  & 0.8114 & 0.4407 & 8.69M
%                         & 0.7659 & 0.3930 & 35.43M & 0.7759 & 0.3837 & 35.43M          \\   
% & Taylor$\dagger$     & \textbf{0.8107} & \textbf{0.4412} & 8.69M & \textbf{0.8116} & \textbf{0.4404} & 8.69M
%                         & \underline{0.7708} & 0.3874 & 35.43M & 0.7772 & 0.3819 & 35.43M          \\ 
\cline{2-14}
& Shaver-Zero           & 0.8101 & 0.4417 & 8.69M  & 0.8114 & 0.4407 & 8.69M
                        & 0.7655 & 0.3934 & 35.43M & 0.7759 & 0.3837 & 35.43M          \\
& Shaver-Zero$\dagger$  & 0.8103 & 0.4415 & 8.69M & \textbf{0.8116} & \textbf{0.4404} & 8.69M
                        & \textbf{0.7715} & \textbf{0.3855} & 35.43M & \underline{0.7777} & \underline{0.3817} & 35.43M          \\                        
& Shaver-Codebook       & 0.8101 & 0.4417 & 8.69M  & 0.8114 & 0.4407 & 8.69M
                        & 0.7647 & 0.3939 & 35.43M & 0.7762 & 0.3838 & 35.43M          \\
& Shaver-Codebook$\dagger$   & \textbf{0.8105} & \textbf{0.4414} & 8.69M & \underline{0.8115} & \underline{0.4405} & 8.69M
                        & 0.7644 & 0.3903 & 35.43M & \textbf{0.7781} & \textbf{0.3816} & 35.43M          \\                        
                      
\cline{1-14}
\multirow{12}{*}{$\sim 80\%$} 
& QR \cite{qr2019}       & 0.8078       & 0.4438 & 3.48M & 0.8091 & 0.4427 & 3.48M
                        & \underline{0.7695} & \underline{0.3871} & 14.17M & 0.7698 & 0.3922 & 14.17M \\
& TTRec \cite{ttrec2021} & 0.8070       & 0.4446 & 3.15M & 0.8103 & 0.4416 & 3.48M
                        & 0.7651 & 0.3902 & 14.17M & 0.7710 & 0.3900 & 14.17M            \\
& DHE \cite{dhe2021}     & 0.8053       & 0.4463 & 3.17M & 0.8109 & 0.4412 & 3.17M
                        & 0.7536 & 0.3957 & 14.74M & 0.7650 & 0.3916 & 14.74M           \\
& PEP \cite{pep2021}  & 0.8098 & 0.4419 & 3.47M & 0.8108 & 0.4413 & 3.46M
                         & 0.7633  & 0.3896 & 14.07M & 0.7669 & 0.3906 & 12.57M           \\
& OptEmb \cite{optembed2022}     & 0.8088 & 0.4430 & 3.17M & 0.8112 & 0.4408 & 1.45M 
                        & 0.7585 & 0.3936 & 3.41M & 0.7663 & 0.3877 & 13.24M             \\
& CERP \cite{cerp2023}   & 0.8095 & 0.4423 & 3.21M & 0.8106 & 0.4416 & 3.44M
                        & 0.7638 & 0.3892 & 14.14M & 0.7673 & 0.3873 & 13.05M          \\
& MagPrune \cite{tran2024thorough}             & 0.8101 & 0.4417 & 3.48M & 0.8111 & 0.4410 & 3.48M
                         & 0.7604  & 0.3962 & 14.17M & 0.7713 & 0.3862 & 14.17M           \\

% & Taylor                & 0.8101 & 0.4417 & 3.48M  & 0.8113 & \underline{0.4407} & 3.48M
%                         & 0.7639 & 0.3936 & 14.17M & 0.7730 & 0.3848 & 14.17M          \\   
% & Taylor$\dagger$     & \textbf{0.8105} & \textbf{0.4413} & 3.48M & \textbf{0.8114} & \textbf{0.4406} & 3.48M
%                         & 0.7649 & 0.3915 & 14.17M & 0.7741 & \textbf{0.3835} & 14.17M          \\ 
\cline{2-14}
& Shaver-Zero           & 0.8100 & 0.4418 & 3.48M  & \textbf{0.8114} & \textbf{0.4407} & 3.48M
                        & 0.7645 & 0.3942 & 14.17M & \underline{0.7745} & \textbf{0.3840} & 14.17M          \\   
& Shaver-Zero$\dagger$  & \textbf{0.8105} & \textbf{0.4414} & 3.48M & \textbf{0.8114} & \textbf{0.4407} & 3.48M
                        & \textbf{0.7715} & \textbf{0.3857} & 14.17M & 0.7735 & 0.3849 & 14.17M          \\ 
& Shaver-Codebook       & 0.8101 & 0.4418 & 3.48M  & \textbf{0.8114} & \textbf{0.4407} & 3.48M
                        & 0.7623 & 0.3952 & 14.17M & \textbf{0.7749} & \underline{0.3842} & 14.17M          \\   
& Shaver-Codebook$\dagger$     & \textbf{0.8105} & \textbf{0.4414} & 3.48M & \textbf{0.8114} & \textbf{0.4407} & 3.48M
                        & 0.7602 & 0.3940 & 14.17M & 0.7717 & 0.3870 & 14.17M          \\ 
\cline{1-14}   
\multirow{12}{*}{$\sim 95\%$} 
& QR \cite{qr2019}       & 0.8033 & 0.4482 & 870K & 0.8064 & 0.4452 & 870K
                        & \underline{0.7644} & \underline{0.3905} & 3.54M & 0.7652 & 0.3895 & 3.54M           \\
& TTRec \cite{ttrec2021} & 0.8087 & 0.4431  & 870K & 0.8106 & 0.4414 & 870K
                        & 0.7608 & 0.3924 &  3.54M & 0.7678 & 0.3903 &  3.54M         \\
& DHE \cite{dhe2021}     & 0.8050 & 0.4466 & 846K & 0.8098 & 0.4420 & 846K 
                        & 0.7601 & 0.3964 & 3.35M & 0.7677 & 0.3913 &  3.35M          \\
& PEP \cite{pep2021}     & 0.8084 & 0.4432  & 806K & \textbf{0.8114} & \textbf{0.4406} & 831K  
                        & 0.7590 & 0.3922 & 3.50M & 0.7564 & 0.3938 & 3.52M             \\
& OptEmb \cite{optembed2022}      & 0.8043 & 0.4471 & 863K  & 0.8109 & \underline{0.4408} & 856K
                        & 0.7585 & 0.3936 & 3.41M & 0.7683 & 0.3895 & 3.43M  \\
& CERP \cite{cerp2023}   & 0.8062  & 0.4454  & 864K & 0.8107 & 0.4414 & 850K
                        & 0.7607 & 0.3920 & 3.54M & 0.7631 & 0.3933 & 3.54M          \\
& MagPrune \cite{tran2024thorough}              & 0.8080 & 0.4436  & 869K & 0.8086 & 0.4434 & 869K 
                        & 0.7501    & 0.4034 & 3.54M & 0.7602 & 0.3924 & 3.54M        \\
% & Taylor                & 0.8092 & 0.4425 & 869K  & 0.8107 & 0.4414 & 869K
%                         & 0.7524 & 0.4000 & 3.54M & 0.7641 & 0.3891 & 3.54M          \\
% & Taylor$\dagger$     & 0.8102 & 0.4416 & 869K & 0.8110 & 0.4410 & 869K
%                         & 0.7614 & 0.3931 & 3.54M & 0.7679 & 0.3872 & 3.54M          \\
\cline{2-14}
& Shaver-Zero           & 0.8085 & 0.4432 & 869K  & 0.8110 & 0.4412 & 869K
                        & 0.7575 & 0.3984 & 3.54M & \underline{0.7690} & \textbf{0.3865} & 3.54M          \\
& Shaver-Zero$\dagger$  & \underline{0.8104} & \underline{0.4414} & 869K & \underline{0.8112} & 0.4409 & 869K
                        & \textbf{0.7655} & \textbf{0.3902} & 3.54M & \textbf{0.7703} & \underline{0.3868} & 3.54M          \\
& Shaver-Codebook       & 0.8093 & 0.4425 & 870K  & \underline{0.8112} & 0.4410 & 870K
                        & 0.7543 & 0.4002 & 3.54M & 0.7683 & 0.3873 & 3.54M          \\
& Shaver-Codebook$\dagger$     & \textbf{0.8106} & \textbf{0.4413} & 870K & \underline{0.8112} & 0.4410 & 870K
                        & 0.7552 & 0.3974 & 3.54M & 0.7670 & 0.3952 & 3.54M          \\
\hline 
\end{tabular}
    \label{tab:deepfm-exp-result}
\end{table*}

==> figures/rq1/performance-table-v2.tex <==
\begin{table*}
    \centering
\renewcommand{\arraystretch}{1.2}
\setlength\tabcolsep{4pt}
\caption{Results on CTR prediction with DeepFM and DCN as the base models. The sparsity $t$ indicates the number of pruned parameters (the higher $t$ is, the more parameters are reduced). \#Para indicates the parameter size of the embedding table (M: million, K: thousand). $\dagger$ denotes fine-tuned models after pruned. In each column, the best result is marked in bold and the second best one is underlined.}
\vspace{-0.2cm}


% |Backbone|Method|50%|||80%|||95%|||
% ||AUC|LogLoss|Params|AUC|LogLoss|Params|AUC|LogLoss|Params|
\begin{tabular}{cl|llr|llr|llr}
\hline
&   & \multicolumn{3}{c|}{50\%} &  \multicolumn{3}{c|}{80\%} &  \multicolumn{3}{c}{95\%} \\
& Method & AUC & Loss & \#Params & AUC & Loss & \#Params & AUC & Loss & \#Params \\
\hline
\end{tabular}
\end{table*}




==> figures/rq1/performance-table.tex <==
\begin{table*}[t!]
    \centering
\renewcommand{\arraystretch}{1.2}
\setlength\tabcolsep{4pt}
\caption{Results on CTR prediction with DeepFM and DCN as the base models. The sparsity $t$ indicates the number of pruned parameters (the higher $t$ is, the more parameters are reduced). \#Para indicates the parameter size of the embedding table (M: million, K: thousand). $\dagger$ denotes fine-tuned models after pruned. In each column, the best result is marked in bold and the second best one is underlined.}
\vspace{-0.2cm}
\begin{tabular}{cl|llr|llr||llr|llr}
\hline
    & & \multicolumn{6}{c||}{Criteo} & \multicolumn{6}{c}{Avazu} \\
\cline{3-14}
    & & \multicolumn{3}{c|}{DeepFM} & \multicolumn{3}{c||}{DCN} & \multicolumn{3}{c|}{DeepFM} & \multicolumn{3}{c}{DCN} \\
\cline{3-14}
     Sparsity    & Method &  AUC      & Loss & \#Para  &  AUC      & Loss & \#Para  & AUC      & Loss & \#Para &  AUC      & Loss & \#Para \\
\cline{1-14}
    0\% & Original & 0.8102 & 0.4416 & 17.39M & 0.8114 & 0.4407 & 17.39M 
                   & 0.7658 & 0.3932 & 70.86M & 0.7759 & 0.3839 & 70.86M \\
\cline{1-14}
 -\% & OptEmb & 0.8088 & 0.4429 & 4.41M & 0.8112 & 0.4408 & 1.45M 
                & 0.7585 & 0.3936 & 3.41M & 0.7671 & 0.3878 & 19.81M \\
\cline{1-14}
\multirow{12}{*}{$\sim 50\%$} % update 6 to 6 + 6 = 12
& QR\cite{qr2019}       & 0.8081  & 0.4435 & 8.69M & 0.8095 & 0.4425 & 8.69M 
                        & 0.7697  & \underline{0.3864} & 35.43M & 0.7743 & 0.3857 & 35.43M           \\
& TTRec\cite{ttrec2021} & 0.8075  & 0.4442 & 9.36M & 0.8112 & 0.4408 & 8.26M
                        & 0.7647  & 0.3915 & 35.43M & 0.7711 & 0.3873 & 35.43M         \\
& DHE\cite{dhe2021}     & 0.8050  & 0.4467 & 8.69M & 0.8095 & 0.4427 & 8.69M
                        & 0.7554  & 0.3959 & 31.74M & 0.7594 & 0.3921 & 31.74M         \\
& PEP\cite{pep2021}     & \underline{0.8105} & \underline{0.4414} & 8.67M & 0.8113 & 0.4407 & 8.69M
                        & 0.7647 & 0.3886  & 29.67M  & 0.7754 & 0.3852 & 33.55M      \\
& CERP\cite{cerp2023}   & 0.8099  & 0.4419  & 8.66M  & 0.8110 & 0.4410 & 8.66M       
                        & 0.7649 & 0.3885 & 35.30M & 0.7723 & 0.3852 & 35.34M     \\
& MagPrune              & 0.8102  & 0.4417 & 8.69M & 0.8113 & 0.4407 & 8.69M
                        & 0.7655  & 0.3932 & 35.43M & 0.7754 & 0.3841 & 35.43M          \\
& Taylor                & 0.8102 & 0.4416 & 8.69M  & 0.8114 & 0.4407 & 8.69M
                        & 0.7659 & 0.3930 & 35.43M & 0.7759 & 0.3837 & 35.43M          \\   
& Taylor$\dagger$     & \textbf{0.8107} & \textbf{0.4412} & 8.69M & \textbf{0.8116} & \textbf{0.4404} & 8.69M
                        & \underline{0.7708} & 0.3874 & 35.43M & 0.7772 & 0.3819 & 35.43M          \\ 
\cline{2-14}
& Shaver-Zero           & 0.8101 & 0.4417 & 8.69M  & 0.8114 & 0.4407 & 8.69M
                        & 0.7655 & 0.3934 & 35.43M & 0.7759 & 0.3837 & 35.43M          \\
& Shaver-Zero$\dagger$  & 0.8103 & 0.4415 & 8.69M & \textbf{0.8116} & \textbf{0.4404} & 8.69M
                        & \textbf{0.7715} & \textbf{0.3855} & 35.43M & \underline{0.7777} & \underline{0.3817} & 35.43M          \\                        
& Shaver-Codebook       & 0.8101 & 0.4417 & 8.69M  & 0.8114 & 0.4407 & 8.69M
                        & 0.7647 & 0.3939 & 35.43M & 0.7762 & 0.3838 & 35.43M          \\
& Shaver-Codebook$\dagger$   & \underline{0.8105} & \underline{0.4414} & 8.69M & 0.8115 & 0.4405 & 8.69M
                        & 0.7644 & 0.3903 & 35.43M & \textbf{0.7781} & \textbf{0.3816} & 35.43M          \\                        
                      
\cline{1-14}
\multirow{12}{*}{$\sim 80\%$} 
& QR\cite{qr2019}       & 0.8078       & 0.4438 & 3.48M & 0.8091 & 0.4427 & 3.48M
                        & \underline{0.7695} & \underline{0.3871} & 14.17M & 0.7698 & 0.3922 & 14.17M \\
& TTRec\cite{ttrec2021} & 0.8070       & 0.4446 & 3.15M & 0.8103 & 0.4416 & 3.48M
                        & 0.7651 & 0.3902 & 14.17M & 0.7710 & 0.3900 & 14.17M            \\
& DHE\cite{dhe2021}     & 0.8053       & 0.4463 & 3.17M & 0.8109 & 0.4412 & 3.17M
                        & 0.7536 & 0.3957 & 14.74M & 0.7650 & 0.3916 & 14.74M           \\
& PEP\cite{pep2021}  & 0.8098 & 0.4419 & 3.47M & 0.8108 & 0.4413 & 3.46M
                         & 0.7633  & 0.3896 & 14.07M & 0.7669 & 0.3906 & 12.57M           \\
& OptEmb\cite{optembed2022}     & 0.8088 & 0.4430 & 3.17M & 0.8112 & 0.4408 & 1.45M 
                        & 0.7585 & 0.3936 & 3.41M & 0.7663 & 0.3877 & 13.24M             \\
& CERP\cite{cerp2023}   & 0.8095 & 0.4423 & 3.21M & 0.8106 & 0.4416 & 3.44M
                        & 0.7638 & 0.3892 & 14.14M & 0.7673 & 0.3873 & 13.05M          \\
& MagPrune\cite{tran2024thorough}              & 0.8101 & 0.4417 & 3.48M & 0.8111 & 0.4410 & 3.48M
                         & 0.7604  & 0.3962 & 14.17M & 0.7713 & 0.3862 & 14.17M           \\

& Taylor                & 0.8101 & 0.4417 & 3.48M  & 0.8113 & \underline{0.4407} & 3.48M
                        & 0.7639 & 0.3936 & 14.17M & 0.7730 & 0.3848 & 14.17M          \\   
& Taylor$\dagger$     & \textbf{0.8105} & \textbf{0.4413} & 3.48M & \textbf{0.8114} & \textbf{0.4406} & 3.48M
                        & 0.7649 & 0.3915 & 14.17M & 0.7741 & \textbf{0.3835} & 14.17M          \\ 
\cline{2-14}
& Shaver-Zero           & 0.8100 & 0.4418 & 3.48M  & \textbf{0.8114} & \underline{0.4407} & 3.48M
                        & 0.7645 & 0.3942 & 14.17M & \underline{0.7745} & \underline{0.3840} & 14.17M          \\   
& Shaver-Zero$\dagger$  & \textbf{0.8105} & \underline{0.4414} & 3.48M & \textbf{0.8114} & \underline{0.4407} & 3.48M
                        & \textbf{0.7715} & \textbf{0.3857} & 14.17M & 0.7735 & 0.3849 & 14.17M          \\ 
& Shaver-Codebook       & 0.8101 & 0.4418 & 3.48M  & \textbf{0.8114} & \underline{0.4407} & 3.48M
                        & 0.7623 & 0.3952 & 14.17M & \textbf{0.7749} & 0.3842 & 14.17M          \\   
& Shaver-Codebook$\dagger$     & \textbf{0.8105} & \underline{0.4414} & 3.48M & \textbf{0.8114} & \underline{0.4407} & 3.48M
                        & 0.7602 & 0.3940 & 14.17M & 0.7717 & 0.3870 & 14.17M          \\ 
\cline{1-14}   
\multirow{12}{*}{$\sim 95\%$} 
& QR\cite{qr2019}       & 0.8033 & 0.4482 & 870K & 0.8064 & 0.4452 & 870K
                        & \underline{0.7644} & \underline{0.3905} & 3.54M & 0.7652 & 0.3895 & 3.54M           \\
& TTRec\cite{ttrec2021} & 0.8087 & 0.4431  & 870K & 0.8106 & 0.4414 & 870K
                        & 0.7608 & 0.3924 &  3.54M & 0.7678 & 0.3903 &  3.54M         \\
& DHE\cite{dhe2021}     & 0.8050 & 0.4466 & 846K & 0.8098 & 0.4420 & 846K 
                        & 0.7601 & 0.3964 & 3.35M & 0.7677 & 0.3913 &  3.35M          \\
& PEP\cite{pep2021}     & 0.8084 & 0.4432  & 806K & \textbf{0.8114} & \textbf{0.4406} & 831K  
                        & 0.7590 & 0.3922 & 3.50M & 0.7564 & 0.3938 & 3.52M             \\
& OptEmb\cite{optembed2022}      & 0.8043 & 0.4471 & 863K  & 0.8109 & \underline{0.4408} & 856K
                        & 0.7585 & 0.3936 & 3.41M & 0.7683 & 0.3895 & 3.43M  \\
& CERP\cite{cerp2023}   & 0.8062  & 0.4454  & 864K & 0.8107 & 0.4414 & 850K
                        & 0.7607 & 0.3920 & 3.54M & 0.7631 & 0.3933 & 3.54M          \\
& MagPrune\cite{tran2024thorough}              & 0.8080 & 0.4436  & 869K & 0.8086 & 0.4434 & 869K 
                        & 0.7501    & 0.4034 & 3.54M & 0.7602 & 0.3924 & 3.54M        \\
& Taylor\cite{taylor2017}                & 0.8092 & 0.4425 & 869K  & 0.8107 & 0.4414 & 869K
                        & 0.7524 & 0.4000 & 3.54M & 0.7641 & 0.3891 & 3.54M          \\
& Taylor\cite{taylor2017}$\dagger$     & 0.8102 & 0.4416 & 869K & 0.8110 & 0.4410 & 869K
                        & 0.7614 & 0.3931 & 3.54M & 0.7679 & 0.3872 & 3.54M          \\
\cline{2-14}
& Shaver-Zero           & 0.8085 & 0.4432 & 869K  & 0.8110 & 0.4412 & 869K
                        & 0.7575 & 0.3984 & 3.54M & \underline{0.7690} & \textbf{0.3865} & 3.54M          \\
& Shaver-Zero$\dagger$  & \underline{0.8104} & \underline{0.4414} & 869K & \underline{0.8112} & 0.4409 & 869K
                        & \textbf{0.7655} & \textbf{0.3902} & 3.54M & \textbf{0.7703} & \underline{0.3868} & 3.54M          \\
& Shaver-Codebook       & 0.8093 & 0.4425 & 870K  & \underline{0.8112} & 0.4410 & 870K
                        & 0.7543 & 0.4002 & 3.54M & 0.7683 & 0.3873 & 3.54M          \\
& Shaver-Codebook$\dagger$     & \textbf{0.8106} & \textbf{0.4413} & 870K & \underline{0.8112} & 0.4410 & 870K
                        & 0.7552 & 0.3974 & 3.54M & 0.7670 & 0.3952 & 3.54M          \\
\hline 
\end{tabular}
    \label{tab:deepfm-exp-result}
\end{table*}
